Learning from Long-Tailed Noisy Data with Sample Selection and Balanced Loss

The success of deep learning depends on large-scale and well-curated training data, while data in real-world applications are commonly long-tailed and noisy. Many methods have been proposed to deal with long-tailed data or noisy data, while a few methods are developed to tackle long-tailed noisy data. To solve this, we propose a robust method for learning from long-tailed noisy data with sample selection and balanced loss. Specifically, we separate the noisy training data into clean labeled set and unlabeled set with sample selection, and train the deep neural network in a semi-supervised manner with a balanced loss based on model bias. Extensive experiments on benchmarks demonstrate that our method outperforms existing state-of-the-art methods.

==> algorithm/MixMatch.tex <==
\begin{algorithm}[htbp]
    \caption{MixMatch}
    \label{algorithm2}

    \begin{algorithmic}[1]
    \REQUIRE Batch size B, samples with label $\mathcal{L}=\{(x_b, y_b)\}_{b=1}^B$, samples without labels $\mathcal{U}=\{u_b\}_{b=1}^B$, sharpening temperature T, number of augmentations M.
    
    \FOR{b = 1 to B}
        \FOR{m = 1 to M}
            \STATE $\hat{x}_{b, m} = Augment(x_b)$
            \STATE $\hat{u}_{b, m} = Augment(u_b)$
        \ENDFOR
        \STATE $\bar{q}_b = \frac{1}{M}\sum_{m=1}^M$ Softmax $f(\hat{u}_{b, m};\theta^{(k)})$
        \STATE $q_b$ = Sharpen$(\bar{q}_b, T)$
    \ENDFOR
    
    \STATE $\hat{\mathcal{L}} = \{(\hat{x}_{b, m}, y_b)|b \in \{1,...,B\}, m \in \{1,...,M\}\}$
    \STATE $\hat{\mathcal{U}} = \{(\hat{u}_{b, m}, q_b)|b \in \{1,...,B\}, m \in \{1,...,M\}\}$
    \STATE $\mathcal{W}$ = Shuffle(Concat$(\hat{\mathcal{L}}, \hat{\mathcal{U}})$)
    \STATE $\mathcal{L}'$ = \{MixUp$(\hat{\mathcal{L}}_i, \mathcal{W}_i) | i \in \{1,...,|\hat{\mathcal{L}}|\}$\}
    \STATE $\mathcal{U}'$ = \{MixUp$(\hat{\mathcal{U}}_i, \mathcal{W}_{i+|\hat{\mathcal{L}}|}) | i \in \{1,...,|\hat{\mathcal{U}}|\}$\}
    
    \RETURN processed labeled samples $\mathcal{L}'$, processed unlabeled samples $\mathcal{U}'$.

    \end{algorithmic}
\end{algorithm}

==> algorithm/main_nocomment.tex <==
\floatname{algorithm}{Algorithm}


\begin{algorithm}[H]
    
    
    \renewcommand{\thealgorithm}{1}
    \caption{Learning with class-aware Sample Selection and Balanced Loss (SSBL).}
    \label{main1}
    

    \begin{algorithmic}[1]
        \Require Deep neural network $f(\cdot; \theta)$, training dataset $(\mathcal{X}, \mathcal{Y})$, total training epochs $T$, model bias estimation epochs $E$, unsupervised loss weight $\lambda_u$, regularization term weight $\lambda_{reg}$, hyper-parameter of EMA $\sigma$.
        
        \State $\theta$ = WarmUp$(\mathcal{X}, \mathcal{Y}, \theta)$
        \State $\bar{M} = {\{0\}}^{C\times C}$
        \While{$e < E$}
            \State $M^e = {\{0\}}^{C \times C}$
            \State ($\mathcal{L}, \mathcal{U}$) = CASS($\mathcal{X}, \mathcal{Y}, \theta$)
            \For{iter = 1 to num\_iters}
                \State Draw a mini-batch $\mathcal{L}_B = \{(\bm x_b, \tilde{y}_b)|b \in \{1,...,B\}\}$ from $\mathcal{L}$
                \State Draw a mini-batch $\mathcal{U}_B = \{\bm u_b|b \in \{1,...,B\}\}$ from $\mathcal{U}$
                
                \For{c = 1 to C}
                    \State Draw $\mathcal{L}_{B, c} = \{(\bm x, \tilde{y})|(\bm x, \tilde{y}) \in \mathcal{L}_{B}\land \tilde{y} = c\}$ from $\mathcal{L}_{B}$
                    \State $M^e_c = M^e_c + \sum_{(\bm x, \tilde{y}) \in \mathcal{L}_{B, c}}$ Softmax$(f(\bm x; \theta))$
                \EndFor
                
                \State ($\mathcal{L}', \mathcal{U}'$) = $\text{MixMatch}_{M}$$(\mathcal{L}_B, \mathcal{U}_B)$
                \State $L_\mathcal{L}, L_\mathcal{U}$ = SoftmaxCE$(\mathcal{L}'; \theta)$, SoftmaxMSE$(\mathcal{U}'; \theta)$
                \State $L = L_\mathcal{L} + \lambda_u L_\mathcal{U} + \lambda_{reg} L_{reg}$
                \State $\theta = SGD(L, \theta)$
            \EndFor
            \State Normalize $M^e$
            \State $\bar{M} = \sigma \bar{M} + (1-\sigma) M^e$
        \EndWhile
        
        \State $R_{ij} = \frac{\bar{M}_{ij}}{\bar{M}_{ji}}, R \in \mathbb{R}^{C \times C}$ 
        
        \While{$e < T$}
            \State ($\mathcal{L}, \mathcal{U}$) = CASS($\mathcal{X}, \mathcal{Y}, \theta$)
            \For{iter = 1 to num\_iters}
                \State Draw a mini-batch $\mathcal{L}_B = \{(\bm x_b, \tilde{y}_b)|b \in \{1,...,B\}\}$ from $\mathcal{L}$
                \State Draw a mini-batch $\mathcal{U}_B = \{\bm u_b|b \in \{1,...,B\}\}$ from $\mathcal{U}$
                
                \State ($\mathcal{L}', \mathcal{U}'$) = $\text{MixMatch}_{M}$$(\mathcal{L}_B, \mathcal{U}_B)$
                \State $L'_\mathcal{L}, L_\mathcal{U} = L_{\bm \alpha}(\mathcal{L}'; \theta, R)$, SoftmaxMSE$(\mathcal{U}'; \theta)$
                \State $L = L'_\mathcal{L} + \lambda_u L_\mathcal{U} + \lambda_{reg} L_{reg}$
                \State $\theta = SGD(L, \theta)$
            \EndFor
        \EndWhile
        

    \end{algorithmic}
    
\end{algorithm}


==> figure/accuracy_ce_cb.tex <==
\begin{figure}
    \centering
    \subfigure[$\rho$=100.]{
    \begin{minipage}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=4.5cm]{images/cifar-10-100-sample.pdf}
    \end{minipage}
    }
    \hspace{.1in}
    \subfigure[$\rho$=50.]{
    \begin{minipage}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=4.5cm]{images/cifar-10-50-sample.pdf}
    \end{minipage}
    }
    \hspace{.1in}
    \subfigure[$\rho$=10.]{
    \begin{minipage}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=4.5cm]{images/cifar-10-10-sample.pdf}
    \end{minipage}
    }
    \captionsetup{skip=0pt}   
    \caption{Comparison between ERM and CB loss in test accuracy (\%) on long-tailed CIFAR-10, where $\rho \in \{100, 50, 10\}$. For ERM, the model's test accuracy of class 5 is consistently lower than that of class 6, even though the training data is biased to class 5. For CB loss, a long-tailed method based on the data bias, the model's test accuracy of class 5 is lower than that of class 8 when $\rho \in \{50, 10\}$, indicating the discrepancy between the model bias and the data bias.}
    \label{model bias}
\end{figure}

==> figure/precision_recall.tex <==
\begin{figure}[t]
% \vspace{-0.2cm}
    \centering
    \includegraphics[width=240pt]{images/precision_cifar100_0.01_0.5_.pdf}
    \includegraphics[width=240pt]{images/recall_cifar100_0.01_0.5_.pdf}
    \captionsetup{skip=5pt}
    % \vspace{-0.2cm}
    \caption{Comparison of precision and recall between class-aware sample selection and sample selection with single GMM. We visualize the precision and recall of samples selected as clean for all and three splits of classes: Many (more than 100 images), Medium (20$\sim$100 images) and Few (less than 20 images). The experiment is conducted on long-tailed CIFAR-100 with symmetric noise. The imbalance ratio $\rho=100$ and the noise rate $r=0.5$, which is an extremely hard setting.}
    % \vspace{-0.4cm}
    \label{pr}
\end{figure}

==> figure/workflow.tex <==
\begin{figure}
    \centering
    \includegraphics[width=13cm]{images/overview_0515.pdf}
    \captionsetup{skip=0pt}   
    \caption{Workflow of the model bias estimation stage and the symmetrical balance stage.}
    \label{workflow}
\end{figure}

==> table/animal10n.tex <==
\begin{table}[ht]
\tiny

%\vspace{-0.2cm}
    \centering
    \resizebox{200pt}{!}{
    \begin{tabular}{l|c c c}
    \toprule
    {Imbalance Ratio} & {20} & {50} & {100} \\
    \hline
    {H2E \citep{yi2022identifying}} & {77.04} & {74.94} & {66.58} \\
    \hline
    {SSBL} & {80.20} & {75.06} & {68.20} \\
    \hline
    {SSBL+RandAug} & \textbf{81.58} & \textbf{78.82} & \textbf{71.84} \\
    \hline
    \hline
    {DivideMix-LA} & {79.10} & {75.58} & {69.06} \\
    \hline
    {DivideMix-DRW} & {78.96} & {71.68} & {68.14} \\
    \hline
    {$\text{SSBL}_2$} & \textbf{81.20} & \textbf{75.84} & \textbf{69.20} \\
    \bottomrule
    \end{tabular}
    }
    
    \vspace{-0.3cm}
    \caption{Comparison with baselines in test accuracy (\%) on long-tailed versions of Animal-10N with real-world noise. $\text{SSBL}$ represents our performance of single model, while $\text{SSBL}_2$ represents our ensemble performance of two models. Results of H2E are borrowed from its original paper.}
    \label{animal10n}
    \vspace{-0.5cm}
\end{table}

==> table/cifar-asym-all.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[ht] 
\huge

\vspace{-0.2cm}
    \centering
    \resizebox{400pt}{!}{%
    \begin{tabular}{c|c c c|c c c|c c c}
    \toprule
    {Imbalance Ratio} & \multicolumn{3}{c|}{10}    & \multicolumn{3}{c|}{50}    & \multicolumn{3}{c}{100} \\
    \hline
    {Cls.} & {Noisy\&Rare} & {Clean} & {All} & {Noisy\&Rare} & {Clean} & {All} & {Noisy\&Rare} & {Clean} & {All} \\
    \hline
    {ERM} &  {49.35} &  \textbf{96.18} & {77.45} & {32.88} &  {96.43} & {71.01} &  {28.13} &  \textbf{96.25} & {69.00} \\
     \hline
    %{LDAM-DRW} & {53.88} & {92.85} & {35.48} & {93.45} & {37.90} & {93.53} \\
    %\hline
    %{LA} & {62.70} & {94.12} & {50.13} & {93.57} & {50.18} & {93.75} \\
    %\hline
    {Co-teaching \citep{han2018co}} &  {49.95} &  {95.13} & {77.06} &  {30.30} &  {95.62} & {69.49} &  {24.68} &  {95.78} & {67.34}  \\
    \hline
    {HAR-DRW \citep{cao2020heteroskedastic}} &  {63.38} &  {95.57} & {82.69} &  \textbf{39.08} &  {95.60} & \textbf{72.99} &  {29.58} &  {95.82} & {69.32}  \\
    \hline
    {MW-Net \citep{shu2019meta}} &  {59.60} &  {95.97} & {81.42} &  {37.13} &  \textbf{96.62} & {72.82} &  {28.30} &  {96.00} & {68.92}  \\
    \hline
    {H2E \citep{yi2022identifying}} &  56.05 & 90.63 & 76.80 & 40.18 & 88.03 & 68.89 & 44.65 & 83.70 & 68.08 \\
    \hline
    %{HAR(240)} &  {66.88} &  {95.58} &  {40.48} &  {94.72} &  {28.98} &  {96.25}  \\
    %\hline
    %{Ours} & 72.65	&92.82	&36.80 &94.48	&32.50	&95.58 \\
    %\hline
    %{Ours(2)} & 75.08	&94.23 &36.83 &95.88	&33.00	&96.20 \\
    {Ours} & \textbf{77.58}	&94.75 & \textbf{87.88}	&38.70 &94.35 & {72.09}	&\textbf{33.00}	&94.65 & \textbf{69.99} \\
    \hline
    \hline
    {ELR+ \citep{liu2020early}} & 40.27	&\textbf{96.63} & {74.09}	&25.98 &\textbf{96.57} & {68.33}	&22.57	&\textbf{96.68} & {67.04} \\
    \hline
    {DivideMix \citep{li2020dividemix}} &75.75 & 96.28 & {88.07} & 32.45 & 93.68 & {69.19} & 25.05 & 95.73 & {67.46} \\
    \hline
    {DivideMix-LA} & 66.68 & 95.35 & 83.88 & 38.48 & 94.53 & 72.11 & 24.73 & 94.20 & 66.41 \\
    \hline
    {DivideMix-DRW} & 60.90 & 95.33 & {81.56} & 37.30 & 93.50 & {71.02} & 33.55 & 93.97 & {69.80} \\
    \hline
    {$\text{Ours}_2$} & \textbf{78.90} &95.45 & \textbf{88.83} &\textbf{39.30} &95.93 & \textbf{73.28} &\textbf{34.48} &96.07 & \textbf{71.43} \\
    \bottomrule
    \end{tabular}%
    }
    \vspace{-0.2cm}
    \caption{Comparison with baselines in test accuracy (\%) on step-imbalanced CIFAR-10 with asymmetric noise. $\text{Ours}$ represents our performance of single model, while $\text{Ours}_2$ represents our ensemble performance of two models.}
    \label{cifar-asym-all}%
    \vspace{-0.2cm}
\end{table*}%


==> table/cifar-asym-only-all.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t] 
\large

    % \vspace{-0.2cm}
    \centering
    \resizebox{180pt}{!}{%
    \begin{tabular}{l|c c c}
    \toprule
    {Imbalance Ratio} & {10}  &  {50}   & {100} \\
    \hline
    {ERM} &  {77.45} & {71.01} & {69.00} \\
     \hline
    %{LDAM-DRW} & {53.88} & {92.85} & {35.48} & {93.45} & {37.90} & {93.53} \\
    %\hline
    %{LA} & {62.70} & {94.12} & {50.13} & {93.57} & {50.18} & {93.75} \\
    %\hline
    {Co-teaching \citep{han2018co}} &  {77.06} & {69.49} & {67.34}  \\
    \hline
    {HAR-DRW \citep{cao2020heteroskedastic}} & {82.69} &  {72.17} & {69.32}  \\
    \hline
    {MW-Net \citep{shu2019meta}} & {81.42} & {72.82} & {68.92}  \\
    \hline
    {H2E \citep{yi2022identifying}} & 76.80 &  68.89 &  68.08 \\
    \hline
    %{HAR(240)} &  {66.88} &  {95.58} &  {40.48} &  {94.72} &  {28.98} &  {96.25}  \\
    %\hline
    %{SSBL} & 72.65	&92.82	&36.80 &94.48	&32.50	&95.58 \\
    %\hline
    %{SSBL(2)} & 75.08	&94.23 &36.83 &95.88	&33.00	&96.20 \\
    {SSBL} &  \textbf{87.88}	& \textbf{72.95}	& \textbf{70.16} \\
    \hline
    \hline
    {ELR+ \citep{liu2020early}} & {74.09}	& {68.33}	& {67.04} \\
    \hline
    {DivideMix \citep{li2020dividemix}} & {88.07} & {69.19} & {67.46} \\
    \hline
    {DivideMix-LA} & 83.88 & 72.11 & 66.41 \\
    \hline
    {DivideMix-DRW} & {81.56} & {71.02} & {69.80} \\
    \hline
    {$\text{SSBL}_2$} & \textbf{88.83} & \textbf{73.96} & \textbf{71.43} \\
    \bottomrule
    \end{tabular}%
    }
    % \vspace{-0.3cm}
    \caption{Comparison with baselines in test accuracy (\%) on step-imbalanced versions of CIFAR-10 with asymmetric noise. $\text{SSBL}$ represents our performance of single model, while $\text{SSBL}_2$ represents our ensemble performance of two models.}
    \label{cifar-asym-only-all}%
    \vspace{-0.2cm}
\end{table}%


==> table/cifar-asym.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
    \centering
    \resizebox{400}{!}{%
    \begin{tabular}{c|c c|c c|c c}
    \toprule
    {Imbalance Ratio} & \multicolumn{2}{c|}{10}    & \multicolumn{2}{c|}{50}    & \multicolumn{2}{c}{100} \\
    {Cls.} & {Noisy\&Rare Cls.} & {Clean Cls.} & {Noisy\&Rare Cls.} & {Clean Cls.} & {Noisy\&Rare Cls.} & {Clean Cls.} \\
    \hline
    {ERM} &  {49.35} &  {96.18} &  {32.88} &  {96.43} &  {28.13} &  {96.25} \\
     \hline
    %{LDAM-DRW} & {53.88} & {92.85} & {35.48} & {93.45} & {37.90} & {93.53} \\
    %\hline
    %{LA} & {62.70} & {94.12} & {50.13} & {93.57} & {50.18} & {93.75} \\
    %\hline
    {Co-teaching} &  {00.00} &  {87.68} &  {00.00} &  {83.73} &  {00.00} &  {84.33}  \\
    \hline
    {HAR} &  {63.38} &  {95.57} &  {39.08} &  {95.60} &  {29.58} &  {95.82}  \\
    \hline
    {MW-Net} &  {59.60} &  {95.97} &  {37.13} &  {96.62} &  {28.30} &  {96.00}  \\
    \hline
    %{HAR(240)} &  {66.88} &  {95.58} &  {40.48} &  {94.72} &  {28.98} &  {96.25}  \\
    %\hline
    %{Ours} & 72.65	&92.82	&36.80 &94.48	&32.50	&95.58 \\
    %\hline
    %{Ours(2)} & 75.08	&94.23 &36.83 &95.88	&33.00	&96.20 \\
    {Ours} & 73.53	&93.85	&39.00 &95.38	&31.03	&95.88 \\
    \hline
    \hline
    {ELR+} & 40.27	&96.63	&25.98 &96.57	&22.57	&96.68 \\
    \hline
    {DivideMix} &75.75 & 96.28 & 32.45 & 93.68 & 25.05 & 95.73 \\
    \hline
    {DivideMix-DRW} & 60.90 & 95.33 & 37.30 & 93.50 & 33.55 & 93.97 \\
    \hline
    {$\text{Ours}_2$} & 73.50 &95.93 &38.78 &96.50	&31.78	&96.58 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Comparison with state-of-the-art methods in test accuracy (\%) on step-imbalanced CIFAR-10 with asymmetric noise. $\text{Ours}_2$ represents our ensemble performance of two models.}
    \label{cifar-asym}%
\end{table}%


==> table/clothing1m.tex <==
\begin{table}[ht]
\tiny

%\vspace{-0.2cm}
    \centering
    \resizebox{200pt}{!}{
    \begin{tabular}{l|c|c|c}
    \toprule
    {Imbalance Ratio} & {20} & {50} & {100} \\
    \hline
    {H2E \citep{yi2022identifying}} & {70.41} & {67.81} & {61.58} \\
    \hline
    {SSBL} & \textbf{71.74} & {69.37} & {66.80} \\
    \hline
    {SSBL+RandAug} & {71.66} & \textbf{71.04} & \textbf{67.65} \\
    \hline
    \hline
    {DivideMix-LA} & {71.20} & {70.09} & {67.20} \\
    \hline
    {DivideMix-DRW} & {71.56} & {69.83} & {66.85} \\
    \hline
    {$\text{SSBL}_2$} & \textbf{72.41} & \textbf{70.76} & \textbf{67.91} \\
    \bottomrule
    \end{tabular}
    }
    
    \vspace{-0.2cm}
    \caption{Comparison with baselines in test accuracy (\%) on long-tailed versions of Clothing1M with real-world noise. $\text{SSBL}$ represents our performance of single model, while $\text{SSBL}_2$ represents our ensemble performance of two models.}
    \label{clothing1m}
    \vspace{-0.1cm}
\end{table}

==> table/clothing1m_and_food101n.tex <==
\begin{table}[ht]
\Large

%\vspace{-0.2cm}
    \centering
    \resizebox{250pt}{!}{
    \begin{tabular}{l|c c c|c c c}
    \toprule
    {Dataset} & \multicolumn{3}{c|}{Clothing1M} & \multicolumn{3}{c}{Food-101N} \\
    \hline
    {Imbalance Ratio} & {20} & {50} & {100} & {20} & {50} & {100} \\
    \hline
    {H2E \citep{yi2022identifying}} & {70.41} & {67.81} & {61.58} & {70.35} & {63.69} & {58.66}\\
    \hline
    {SSBL} & \textbf{71.74} & {69.37} & {66.80} & {72.05} & {66.78} & {61.62} \\
    \hline
    {SSBL+RandAug} & {71.66} & \textbf{71.04} & \textbf{67.65} & \textbf{74.06} & \textbf{68.56} & \textbf{64.64} \\
    \hline
    \hline
    {DivideMix-LA} & {71.20} & {70.09} & {67.20} & {} & {} & {} \\
    \hline
    {DivideMix-DRW} & {71.56} & {69.83} & {66.85} & {} & {53.98} & {53.65} \\
    \hline
    {$\text{SSBL}_2$} & \textbf{72.41} & \textbf{70.76} & \textbf{67.91} & \textbf{74.39} & \textbf{69.06} & \textbf{63.67} \\
    \bottomrule
    \end{tabular}
    }
    
    \vspace{-0.3cm}
    \caption{Comparison with baselines in test accuracy (\%) on long-tailed versions of Clothing1M and Food-101N with real-world noise. $\text{SSBL}$ represents our performance of single model, while $\text{SSBL}_2$ represents our ensemble performance of two models. Results of H2E on Food-101N are borrowed from its original paper.}
    \label{clothing1m_and_food101n}
    \vspace{-0.4cm}
\end{table}

==> table/food101n.tex <==
\begin{table}[ht]
\tiny

%\vspace{-0.2cm}
    \centering
    \resizebox{200pt}{!}{
    \begin{tabular}{l|c|c|c}
    \toprule
    {Imbalance Ratio} & {20} & {50} & {100} \\
    \hline
    {H2E \citep{yi2022identifying}} & {70.35} & {63.69} & {58.66} \\
    \hline
    {SSBL} & {72.05} & {66.78} & {61.62} \\
    \hline
    {SSBL+RandAug} & \textbf{74.06} & \textbf{68.56} & \textbf{64.64} \\
    \hline
    \hline
    {DivideMix-LA} & {} & {} & {} \\
    \hline
    {DivideMix-DRW} & {} & {53.98} & {53.65} \\
    \hline
    {$\text{SSBL}_2$} & \textbf{74.39} & \textbf{69.06} & \textbf{63.67} \\
    \bottomrule
    \end{tabular}
    }
    
    \vspace{-0.2cm}
    \caption{Comparison with baselines in test accuracy (\%) on long-tailed versions of Food-101N with real-world noise. $\text{SSBL}$ represents our performance of single model, while $\text{SSBL}_2$ represents our ensemble performance of two models. Results of H2E are borrowed from its original paper.}
    \label{food101n}
    \vspace{-0.1cm}
\end{table}

==> table/gamma.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t] 


\vspace{0.2cm}
    \centering
    \resizebox{200pt}{!}{%
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \multicolumn{2}{c|}{Noise Rate} & \multicolumn{2}{c|}{0.2} & \multicolumn{2}{c}{0.5} \\
    \hline
    \multicolumn{2}{c|}{Imbalance Ratio} & {50} & {100} & {50} & {100} \\
    \hline
    \multirow{2}{*}{$\gamma_{sup} = 3, \gamma_{rel} = 0$} & {Best} & {84.77} & {79.21} & {75.58} & {70.51} \\
    & {Last} & {82.44} & {77.00} & {74.86} & {66.76} \\
    \hline
    \multirow{2}{*}{$\gamma_{sup} = 3, \gamma_{rel} = 0.5$} & {Best} & {85.71} & \textbf{80.73} & {76.48} & {71.93} \\
    & {Last} & {85.01} & \textbf{78.77} & {75.19} & {68.12} \\
    \hline
    \multirow{2}{*}{$\gamma_{sup} = 3, \gamma_{rel} = 1$} & {Best} & \textbf{86.30} & {79.84} & {77.72} & {72.36} \\
    & {Last} & \textbf{85.83} & {78.39} & \textbf{75.76} & {68.44} \\
    \hline
    \multirow{2}{*}{$\gamma_{sup} = 3, \gamma_{rel} = 2$} & {Best} & {79.72} & {73.90} & \textbf{79.08} & {72.79} \\
    & {Last} & {50.70} & {41.86} & {74.54} & {59.28} \\
    \hline
    \multirow{2}{*}{$\gamma_{sup} = 3, \gamma_{rel} = 3$} & {Best} & {79.72} & {73.90} & {78.73} & \textbf{73.22} \\
    & {Last} & {46.29} & {42.03} & {64.68} & {60.22} \\
    \hline
    \multirow{2}{*}{$\gamma_{sup} = 1, \gamma_{rel} = 1$} & {Best} & {85.67} & {80.39} & {75.50} & {69.84} \\
    & {Last} & {85.16} & {78.76} & {73.64} & {67.99} \\
    \hline
    \multirow{2}{*}{$\gamma_{sup} = 2, \gamma_{rel} = 1$} & {Best} & {85.43} & {80.24} & {76.95} & {71.56} \\
    & {Last} & {85.19} & {77.82} & {73.39} & \textbf{68.78} \\
    \hline
    \multirow{2}{*}{$\gamma_{sup} = 4, \gamma_{rel} = 1$} & {Best} & {85.55} & {79.60} & {78.21} & {72.88} \\
    & {Last} & {85.55} & {73.08} & {66.27} & {58.26} \\
    \bottomrule
    \end{tabular}%
    }
    % \vspace{-0.3cm}
    \caption{Ablation study of the hyper-parameters $\gamma_{sup}$ and $\gamma_{rel}$ in test accuracy (\%) on long-tailed CIFAR-10 with symmetric noise.}
    \label{gamma}%
    % \vspace{-0.5cm}
\end{table}%


==> table/mini-imagenet-red.tex <==
\begin{table}[t]
\large

%\vspace{-0.2cm}
    \centering
    \resizebox{250pt}{!}{
    \begin{tabular}{l|c c c|c c c}
    \toprule
    {Noise Rate} & \multicolumn{3}{c|}{0.2} & \multicolumn{3}{c}{0.5} \\
    \hline
    {Imbalance Ratio} & {20} & {50} & {100} & {20} & {50} & {100} \\
    \hline
    {Co-teaching \citep{han2018co}} & {22.72} & {20.09} & {17.05} & {17.97} & {14.74} & {13.86} \\
    \hline
    {HAR-DRW \citep{cao2020heteroskedastic}} & {29.78} & {25.94} & {23.30} & {24.10} & {21.34} & {19.14} \\
    \hline
    {MW-Net \citep{shu2019meta}} & {33.56} & {27.74} & {24.46} & {26.72} & {23.10} & {20.82} \\
    \hline
    {H2E \citep{yi2022identifying}} & {26.26} & {24.56} & {20.82} & {25.76} & {20.50} & {17.80} \\
    \hline
    {SSBL} & {36.02} & {31.38} & {28.20} & {30.04} & {26.36} & {23.98} \\
    \hline
    {SSBL+RandAug} & \textbf{37.52} & \textbf{32.54} & \textbf{29.54} & \textbf{31.14} & \textbf{27.94} & \textbf{25.34} \\
    \hline
    \hline
    {ELR+ \citep{liu2020early}} & {31.86} & {26.33} & {24.39} & {26.23} & {23.30} & {20.61} \\
    \hline
    {DivideMix \citep{li2020dividemix}} & {35.96} & {29.02} & {27.36} & {30.10} & {26.42} & {24.20} \\
    \hline
    {DivideMix-LA} & {37.36} & {32.12} & {29.66} & {32.34} & {28.12} & {24.78} \\
    \hline
    {DivideMix-DRW} & {36.56} & {30.14} & {28.48} & {30.64} & {26.62} & {24.34} \\
    \hline
    {$\text{SSBL}_2$} & \textbf{37.92} & \textbf{32.90} & \textbf{30.74} & \textbf{32.84} & \textbf{29.06} & \textbf{26.26} \\
    \bottomrule
    \end{tabular}
    }
    
    % \vspace{-0.3cm}
    \caption{Comparison with baselines in test accuracy (\%) on long-tailed versions of mini-ImageNet-Red with real-world noise. $\text{SSBL}$ represents our performance of single model, while $\text{SSBL}_2$ represents our ensemble performance of two models.}
    \label{mini-imagenet-red}
    % \vspace{-0.4cm}
\end{table}

==> table/webvision-lt.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
    \toprule
    Dataset & \multicolumn{4}{c|}{WebVision} & \multicolumn{4}{c}{ImageNet} \\
    \hline
    \multirow{2}{*}{Imbalanced Factor} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{50} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c}{50} \\
\cline{2-9}          & \multicolumn{1}{l|}{top1} & \multicolumn{1}{l|}{top5} & \multicolumn{1}{l|}{top1} & \multicolumn{1}{l|}{top5} & \multicolumn{1}{l|}{top1} & \multicolumn{1}{l|}{top5} & \multicolumn{1}{l|}{top1} & \multicolumn{1}{l}{top5} \\
    % \hline
    % CE    &       &       &       &       &       &       &       &  \\
    % \hline
    % CB Loss  & 4.28  & 18.20 & 32.36 & 66.36  & 4.88  & 19.48 & 29.56 & 65.80 \\
    \hline
    LDAM-DRW  & 39.36 & 66.28 & 42.60  & 70.60 & 37.92 & 64.76 & 40.84 & 68.76 \\
    \hline
    LA     & 44.84 & 76.68 & 46.72 & 80.52 & 42.52 & 76.40 & 45.96 & 80.76  \\
    \hline
    DivideMix & 54.80  & 73.76   & 61.40 & 82.12  & 54.60 & 74.96       & 62.08  & 82.64 \\
    \hline
    DivideMix-DRW & 57.44 & 72.76  & 65.20  & 81.44  & 57.76  & 73.68  & 65.40   & 82.36 \\
    % \hline
    % $\text{DivideMix}_{\text{mean}}$ & 54.20  & -   & 60.62 & -  & 52.86 & -       & 60.30  & - \\
    \hline
    $\text{DivideMix-DRW}_{\text{mean}}$ & 56.06 & -  & 62.92  & -  & 55.54  & -  & 62.92   & - \\
    \hline
    $\text{Ours}_{\text{mean}}$  & 63.62  & -   & 67.52  & -  & 61.38  & - & 65.7 & - \\
    
    \hline
    \hline
    Ours  & \textbf{65.00}  & \textbf{86.56}   & \textbf{69.32} &  \textbf{88.76}  & \textbf{63.20}  & \textbf{87.64} & \textbf{67.16} & \textbf{88.84} \\
    \bottomrule
    \end{tabular}%
    \caption{Comparison with state-of-the-art methods in test accuracy (\%) on long-tailed versions of mini WebVision. $(\cdot)_{\text{mean}}$ represents the averaged test accuracy of the ensemble model's experts.}
  \label{webvision-lt}%
\end{table}%


==> table/webvision.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  
    \begin{tabular}{l|c|c|c|c}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{2}{c|}{WebVision} & \multicolumn{2}{c}{ImageNet} \\
\cline{2-5}          & \multicolumn{1}{c|}{top1} & \multicolumn{1}{c|}{top5} & \multicolumn{1}{c|}{top1} & \multicolumn{1}{c}{top5} \\
    \hline
    LDAM-DRW & 55.04 & 79.80  & 52.88  & 78.20 \\
    \hline
    LA    & 55.68   & 84.04  & 53.72 & 83.40  \\
    \hline
    Co-teaching & 63.60  & 85.20  & 61.50  & 84.70 \\
    \hline
    HAR   & 75.50  & 90.70  & 70.30  & 90.00 \\
    \hline
    DivideMix & 77.68 & 92.72 & 75.44  & 92.44 \\
    \hline
    DivideMix-DRW & \textbf{78.28} & \textbf{92.04} & 75.44   & 92.56 \\
    % \hline
    % $\text{DivideMix}_{\text{mean}}$ & 76.02 & - & 73.04  & - \\
    \hline
    $\text{DivideMix-DRW}_{\text{mean}}$ & 76.64 & - & 73.80  & - \\
    \hline
    $\text{Ours}_{\text{mean}}$ & 76.96  & -  &  73.64     & - \\
    \hline
    \hline
    Ours  & 78.00  & 91.92  &  \textbf{75.88}     & \textbf{92.6} \\
    \bottomrule
    \end{tabular}%
    \caption{Comparison with state-of-the-art methods in test accuracy (\%) on mini WebVision. $(\cdot)_{\text{mean}}$ represents the averaged test accuracy of the ensemble model's experts.}
  \label{webvision}%
\end{table}%

